Online Sub-Sampling for Reinforcement Learning with General Function Approximation

Most of the existing works for reinforcement learning (RL) with general function approximation (FA) focus on understanding the statistical complexity or regret bounds. However, the computation complexity of such approaches is far from being understood -- indeed, a simple optimization problem over the function class might be as well intractable. In this paper, we tackle this problem by establishing an efficient online sub-sampling framework that measures the information gain of data points collected by an RL algorithm and uses the measurement to guide exploration. For a value-based method with complexity-bounded function class, we show that the policy only needs to be updated for $\propto\operatorname{poly}\log(K)$ times for running the RL algorithm for $K$ episodes while still achieving a small near-optimal regret bound. In contrast to existing approaches that update the policy for at least $\Omega(K)$ times, our approach drastically reduces the number of optimization calls in solving for a policy. When applied to settings in \cite{wang2020reinforcement} or \cite{jin2021bellman}, we improve the overall time complexity by at least a factor of $K$. Finally, we show the generality of our online sub-sampling technique by applying it to the reward-free RL setting and multi-agent RL setting.

==> discussion.tex <==
\subsection{Practical Impacts} The most direct practical impact is the improvement over \citet{wang2020reinforcement}. A notable drawback of applying the algorithm in \citet{wang2020reinforcement} in practice is its bad computational efficiency. Equipped with our framework, the whole time complexity of the algorithm grows linear in $K$ (under the time cost assumption of the regression oracle, see Remark~\ref{rmk3}), making it more suitable for practical use.

Besides, we remark on two possible usages of our theoretical framework in practice: 

1. In DQN, the agent doesn’t need to train after each step. Instead, it uses experience replay to train on small batches once every $n$ steps, where $n$ is a tuning parameter but is fixed during the entire course of training. Our subsampling approach would introduce an efficient and adaptive approach to adjust $n$ – the network is retrained whenever the policy needs a switch. Note that the bonus function defined in our paper can be implemented for DNN and has been implemented in \citet{feng2021provably}. While this idea needs further experimental verification, we believe our methods can inspire more efficient practical algorithms. 

2. Prioritized experience replay~\citep{schaul2015prioritized} is a widely used technique in off-policy RL algorithms. Although the sensitivity scores used in our paper are intended to compute the exploration bonus and decide policy switches, they can be potentially used as priority scores in the prioritized replay buffer. Similar to the linear leverage score sampling (e.g., \citep{cohen2016online}), such a score may improve the conditioning of the dataset and improve the performance of a neural network. 
\subsection{Limitations and Possible Applications}
\label{limit}
Our current approaches rely heavily on the eluder dimension structures of the function class, i.e., the sub-sampled dataset size can be bounded by a function of the eluder dimension. However, one may understand the structure of the algorithm more generally from an information-theoretical point of view: the algorithm switches the policy when there is sufficient information gained, and the data points causing the information change are important points to be stored. Hence, we believe such an algorithmic structure can be further summarized and abstracted to fit a broader range of settings. The idea of measuring information gain has been further studied in \citet{lu2019information}, which we believe can be integrated with our techniques for sampling. We remark that \citet{dong2020root}, a low-regret version of \citet{jiang2017contextual}, is already low-switching without any modification. Though it doesn't directly use our subsampling procedure, it has a similar implicit mechanism for measuring information gain and controlling policy updates. It would be interesting to see whether our framework can incorporate \citet{foster2021statistical}, which is the most general framework for RL with general FA up to now, subsuming the frameworks of \citet{jiang2017contextual}, \citet{jin2021bellman}, and \citet{du2021bilinear}; but it is not computationally efficient. Another future direction is to generalize our results beyond the pure value-based algorithm, e.g., the actor-critic based algorithm~\citep{feng2021provably}
